MetaQA: Combining Expert Agents for Multi-Skill Question Answering

The recent explosion of question answering (QA) datasets and models has increased the interest in the generalization of models across multiple domains and formats by either training on multiple datasets or by combining multiple models. Despite the promising results of multi-dataset models, some domains or QA formats may require specific architectures, and thus the adaptability of these models might be limited. In addition, current approaches for combining models disregard cues such as question-answer compatibility. In this work, we propose to combine expert agents with a novel, flexible, and training-efficient architecture that considers questions, answer predictions, and answer-prediction confidence scores to select the best answer among a list of answer candidates. Through quantitative and qualitative experiments we show that our model i) creates a collaboration between agents that outperforms previous multi-agent and multi-dataset approaches in both in-domain and out-of-domain scenarios, ii) is highly data-efficient to train, and iii) can be adapted to any QA format. We release our code and a dataset of answer predictions from expert agents for 16 QA datasets to foster future developments of multi-agent systems on https://github.com/UKPLab/MetaQA.

==> sections/discussions.tex <==
In more detail, while TWEAC only attempts to predict the agent trained on the domain of the input question, we aim to retrieve the best answer prediction, even if it comes from a model trained on a completely different dataset. For instance, in DuoRC, our MetaQA selects the in-domain agent only for 43\% of its questions, i.e., most of the questions are assigned to agents that are not trained on DuoRC. \rev{}{We also observe that the gap between MetaQA and TWEAC is larger on extractive QA than on multiple-choice. This is expected due to the multiple-choice dataset choices. Their formats differ considerably, which limits agent collaboration. For instance, BoolQ is the only boolean dataset, and RACE is the only non-commonsense multiple-choice dataset. Even the commonsense datasets have differences limiting agent collaboration (SIQA uses a short context passage while CSQA does not have any context). Yet, even with these limitations, MetaQA outperforms TWEAC in three of the five datasets. Lastly, in NarrativeQA and HybridQA the performance is the same because there is only one agent per dataset.}

==> tables/backup_qualitiative_analysis_table.tex <==
\begin{table*}[t]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{lp{0.35\linewidth}p{0.20\linewidth}p{0.20\linewidth}}
\toprule
\textbf{Dataset} & \textbf{Question}                                       & \centering{\textbf{In-domain Agent}} & \textbf{OOD Agent}  \\\midrule
DuoRC   & Who does Rocky Balboa work for as an enforcer? & \textcolor{red}{Adrian}          & \textcolor{green!70!blue}{Tony Gazzo} (NewsQA Agent) \\
TriviaQA-web & Who played the character Mr Chips in the 2002 TV adaptation of Goodbye Mr Chips                        & \textcolor{red}{Timothy Carroll} & \textcolor{green!70!blue}{MartinClunes} (DuoRC Agent)            \\
SearchQA     & This short story, written around 1820, contains the line "If I can but reach that bridge... I am safe" & \textcolor{red}{Legend}       & \textcolor{green!70!blue}{Legend of Sleepy Hollow} (TriviaQA Agent) \\ \bottomrule
\end{tabular}
}
\end{center}
\caption{Examples of questions where our MetaQA system disregard the in-domain agent due to their incorrect predictions (in red) and selects and an out-of-domain (OOD) agent that returns the right answer (in green).}
\label{table:qual_analysis}
\end{table*}

==> tables/dataset_size.tex <==
\begin{table}[t]
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Train} & \textbf{Validation} & \textbf{Test} \\
\midrule
SQuAD            & 86573          & 5253                & 5254          \\
NewsQA           & 74160          & 2106                & 2106          \\
NQ               & 104071         & 6418                & 6418          \\
HotpotQA         & 72928          & 2950                & 2951          \\
TriviaQA-web     & 61688          & 3892                & 3893          \\
SearchQA         & 117384         & 8490                & 8490          \\
DuoRC            & 58752          & 13111               & 13449         \\
QAMR             & 50615          & 18908               & 18770         \\
RACE             & 87866          & 4887                & 4934          \\
CSQA    & 9741           & 611                 & 610           \\
HellaSWAG        & 39905          & 5021                & 5021          \\
SIQA             & 33410          & 977                 & 977           \\
BoolQ            & 9427           & 1635                & 1635          \\
DROP             & 77409          & 4767                & 4768          \\
NarrativeQA      & 32747          & 3461                & 10557         \\
HybridQA         & 62682          & 1733                & 1733        
\\ \bottomrule
\end{tabular}
\caption{Split sizes of each dataset.}
\label{table:dataset_sizes}
\end{table}

==> tables/datasets_table_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\scalebox{0.7}{
\begin{tabular}{lp{0.6\linewidth}p{0.65\linewidth}}
\toprule
    & \textbf{Dataset} & \textbf{Characteristics}                             \\
\midrule
\parbox[t]{2mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{Extractive}}}      & SQuAD \citep{rajpurkar-etal-2016-squad}        & Crowdsourced questions on Wikipedia                                   \\
                                    & NewsQA \citep{trischler-etal-2017-newsqa}       & Crowdsourced questions about News                                        \\
                                    & HotpotQA \citep{yang-etal-2018-hotpotqa}     & Crowdsourced multi-hop questions on Wikipedia                         \\
                                    & SearchQA \citep{dunn2017searchqa}     & Web Snippets, Trivia questions from J! Archive
    \\
                                    & NQ \citep{kwiatkowski-etal-2019-natural}           & Wikipedia, real user queries on Google Search                   \\
                                    & TriviaQA-web \citep{joshi-etal-2017-triviaqa} & Web Snippets, crowdsorced trivia questions  \\
                                    & QAMR \citep{michael-etal-2018-crowdsourcing}         & Wikipedia, predicate-argument understanding \\
                                    & DuoRC \citep{saha-etal-2018-duorc}        & Movie Plots from IMDb and Wikipedia                                \\
\midrule                    
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Multiple-Choice}}} & RACE \citep{lai-etal-2017-race}        & Exams requiring passage summarization and attitude analysis                                       \\
                                    & CSQA \citep{talmor-etal-2019-commonsenseqa}         & Web Snippets, common-sense reasoning                                 \\
               & BoolQ \citep{clark-etal-2019-boolq}       & Wikipedia, Yes/No questions                          \\                     & HellaSWAG \citep{zellers-etal-2019-hellaswag}    & Completing sentences using common sense   \\
                                    & SIQA \citep{sap-etal-2019-social}         & Common sense in social interactions           \\
                                    
                                    \midrule  
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Abs.}}}     & DROP \citep{dua-etal-2019-drop}         & Wikipedia, numerical reasoning              \\
                                    & NarrativeQA \citep{kocisky-etal-2018-narrativeqa} & Books, Movie Scripts                        \\

                                    \midrule  
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{MM}}}                       & HybridQA \citep{chen-etal-2020-hybridqa}     & Wikipedia tables and paragraphs \\& & \\


\bottomrule
\end{tabular}
}
\caption{Summary of the datasets used. Abs. stands for abstractive and MM for multi-modal.}
\label{table:datasets}

\end{table}

==> tables/dev_set_results.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{F1}  \\
\midrule
SQuAD            & 91.42                \\
NewsQA           & 70.89                 \\
NQ               & 78.45                  \\
HotpotQA         & 80.78                \\
TriviaQA-web     & 77.68                   \\
SearchQA         & 77.78                  \\
DuoRC            & 51.03                \\
QAMR             & 83.69                 \\
RACE             &                    \\
CSQA             &                      \\
HellaSWAG        &                   \\
SIQA             &                      \\
BoolQ            &                    \\
DROP             &                   \\
NarrativeQA      &                   \\
HybridQA         &                  
\\ \bottomrule
\end{tabular}
\caption{Dev set results on the released model.}
\label{table:dataset_sizes}
\end{center}
\end{table}

==> tables/license.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{ll}
\toprule
\textbf{Dataset}       & \textbf{License}      \\
\midrule
MRQA          & MIT          \\
DuoRC         & MIT          \\
QAMR          & MIT          \\
RACE          & NA           \\
CommonSenseQA & NA           \\
HellaSWAG     & MIT          \\
SIQA          & NA           \\
BoolQ         & CC BY-SA 3.0 \\
DROP          & CC BY-SA 4.0 \\
NarrativeQA   & Apache 2.0   \\
HybridQA      & MIT     
\\ \bottomrule
\end{tabular}
\caption{License of each dataset.}
\label{table:license}
\end{center}
\end{table}

